Findings of the LoResMT 2021 Shared Task on COVID and Sign Language for Low-resource Languages

We present the findings of the LoResMT 2021 shared task which focuses on machine translation (MT) of COVID-19 data for both low-resource spoken and sign languages. The organization of this task was conducted as part of the fourth workshop on technologies for machine translation of low resource languages (LoResMT). Parallel corpora is presented and publicly available which includes the following directions: English$\leftrightarrow$Irish, English$\leftrightarrow$Marathi, and Taiwanese Sign language$\leftrightarrow$Traditional Chinese. Training data consists of 8112, 20933 and 128608 segments, respectively. There are additional monolingual data sets for Marathi and English that consist of 21901 segments. The results presented here are based on entries from a total of eight teams. Three teams submitted systems for English$\leftrightarrow$Irish while five teams submitted systems for English$\leftrightarrow$Marathi. Unfortunately, there were no systems submissions for the Taiwanese Sign language$\leftrightarrow$Traditional Chinese task. Maximum system performance was computed using BLEU and follow as 36.0 for English--Irish, 34.6 for Irish--English, 24.2 for English--Marathi, and 31.3 for Marathi--English.

==> removed.tex <==
\section{Task and Evaluation}
\label{sec:task}

\subsection{Open Machine Translation}
\label{subsec:open_machine_translation}
Given the limited availability of resources and the important dialectal, orthographic and domain challenges, we %decided to 
designed our task as an unrestrained machine translation shared task: we called it \emph{open} machine translation to emphasize that participants were free to use any resources they could find. 
%All participating teams were allowed to use any additional dataset or resource for training, on top of the provided collection in our official repository. 
Possible resources could, for instance, include existing or newly created parallel data, dictionaries, tools, or pretrained models. 

%The current task examines translation between Spanish and Amerindian languages in an open-domain setting. In this first edition, we included Ash\'aninka, Aymara, Bribri, Guaran\'i, Otomí, Náhuatl, Quechua, Rar\'amuri, Shipibo-Konibo and Wixarika (into and out of Spanish). 
We invited submissions to two different tracks: Systems in Track 1 were allowed to use the development set as part of the training data, since this is a common practice in the machine translation community. Systems in Track 2 were not allowed to be trained directly on the development set, mimicking a more realistic low-resource setting. 
%Details about the development set are presented in \ref{subsec:dev_and_test_sets}.
%\Manuel{Arturo, can you describe this part?}

\subsection{Primary Evaluation}
\label{subsec:evaluation}
In order to be able to evaluate a large number of systems on all 10 languages, we used automatic metrics for our primary evaluation.
Our main metric, which determined the official ranking of systems, was ChrF \cite{popovic-2015-chrf}. %\gn{In the reported results ChrF is between 0-1 and BLEU is between 0-100. Is there a reason for this discrepancy? If not, I'd suggest 0-100 for all, as it saves a decimal place, making the tables more compact, and is a bit easier to read.}\manuel{Solved}
We made this choice due to certain properties of our languages, such as word boundaries not being standardized for all languages and many languages being polysynthetic, resulting in a small number of words per sentence.
%as to not take into account word boundaries, which for non-standarised and highly morphological languages are not well defined, and vary depending the annotator.
 We further reported BLEU scores \cite{papineni-etal-2002-bleu} for all systems and languages.
%and used the second one as the official metric for ranking 

\subsection{Supplementary Evaluation}
\label{subsec:humanevaluation}
To gain additional insight into the strengths and weaknesses of the top-performing submissions, we further performed a supplementary manual evaluation for two language pairs and a limited number of systems, using a subset of the test set. 

We asked our annotators to provide ratings of system outputs using separate 5-point scales for
adequacy and fluency. The annotation was performed by the translator who created the test datasets. The expert received the source sentence in Spanish, the reference in the indigenous language, and an anonymized system output. In addition to the baseline, we considered the 3 highest ranked systems according to our main metric%besides a baseline model
, and randomly selected 100 sentences for each language. The following were the descriptions of the ratings as provided to the expert annotator in Spanish (translated into English here for convenience):
%choose 100 randomly selected sentences, shuffled the and shuffled them. The evaluation criteria provided to the experts is as following:

\paragraph{Adequacy} The output sentence expresses the meaning of the reference.
\begin{enumerate}
\item Extremely bad: The original meaning is not contained at all.
\item Bad: Some words or phrases allow to guess the content.
\item Neutral.
\item Sufficiently good: The original meaning is understandable, but some parts are unclear or incorrect.
\item Excellent: The meaning of the output is the same as that of the reference.
\end{enumerate}
%Correcto
%La frase logra expresar el significado de la referencia
%1. Extremadamente Malo (No se expresa del todo el significado original).
%2. Malo (Algunas palabras pueden o frases permiten adivinar el significado).
%3. Neutral
%4. Suficientemente Bueno (Se logra leer el significado original, pero algunas partes no están claras o son incorrectas).
%5. Excelente (El significado del enunciado es el mismo que el de la frase original).

\paragraph{Fluency} The output sentence is easily readable and looks like a human-produced text.
\begin{enumerate}
\item Extremely bad: The output text does not belong to the target language.
\item Bad: The output sentence is hardly readable.
\item Neutral.
\item Sufficiently good: The output seems like a human-produced text in the target language, but contains weird mistakes.
\item Excellent: The output seems like a human-produced text in the target language, and is readable without issues.
\end{enumerate}
%Fluido
%La frase suena natural al idioma y se logra leer de manera fácil?
%1. Extremadamente Malo (No, la frase no parece ser de la lengua).
%2. Malo (La frase se lee con gran dificultad).
%3. Neutral
%4. Suficiente (La frase parece ser del idioma, pero contiene algunos errores que no parecen humanos).
%5. Excelente (La frase parece ser escrita por un humano, y se puede leer sin problemas).


%\Manuel{Abteen: can you help us with this part?}

% BLEU \cite{papineni-etal-2002-bleu} 
% ChrF \cite{popovic-2015-chrf}  

\section{Languages and Datasets}
\label{sec:datasets}
%For all languages, the domain of the training data differs from that of the development and test sets, however, development and test sets are taken from the same domain and use the same orthography. None of the development and test sets are tokenized; in contrast, some of the training sets are tokenized. 
In this section, we will present the languages and datasets featured in our shared task. Figure \ref{tab:languages} additionally provides an overview of the languages, their linguistic families, and the number of parallel sentences with Spanish.
\label{subsec:provided_datasets}
\begin{table}[]
    \centering
    \small
    \setlength{\tabcolsep}{2.5pt}
    %\begin{adjustbox}{width=\columnwidth}

    \begin{tabular}{lllrrr}
        \toprule
        \textbf{Language} & \textbf{ISO} & \textbf{Family} & \bf Train &\textbf{Dev} & \textbf{Test} \\ \midrule
        Asháninka & cni & Arawak & 3883 & 883 & 1002\\
        Aymara & aym & Aymaran  & 6531 & 996 & 1003\\
        Bribri & bzd & Chibchan & 7508 & 996 & 1003\\
        Guarani & gn & Tupi-Guarani & 26032 & 995 & 1003\\
        Nahuatl & nah & Uto-Aztecan & 16145 & 672 & 996\\
        Otomí & oto & Oto-Manguean  & 4889 & 599 & 1001\\
        Quechua & quy & Quechuan & 125008 & 996 & 1003\\
        Rarámuri & tar & Uto-Aztecan & 14721 & 995 & 1002 \\
        Shipibo-Konibo & shp & Panoan & 14592 & 996 & 1002\\
        Wixarika & hch & Uto-Aztecan & 8966 & 994 & 1003 \\
        
    \bottomrule
    \end{tabular}
    %\end{adjustbox}
    \caption{The languages featured in the AmericasNLP 2021 Shared Task on OMT, their ISO codes, language families and dataset statistics. For the origins of the datasets, please refer to the text.}
    \label{tab:languages}
\end{table}

\subsection{Development and Test Sets}
\label{subsec:dev_and_test_sets}
For system development and testing, we leveraged individual pairs of parallel sentences from AmericasNLI \cite{ebrahimi2021americasnli}. This dataset is a translation of the Spanish version of XNLI \cite{conneau-etal-2018-xnli} into our 10 indigenous languages. It was not publicly available until after the conclusion of the competition, avoiding an accidental inclusion of the test set into the training data by the participants. For more information regarding the creation of the dataset, we refer the reader to \cite{ebrahimi2021americasnli}.

\subsection{Training Data}
%The datasets used for training were collected from previously published parallel datasets.
We collected publicly available datasets in all 10 languages and provided them to the shared task participants as a starting point. We will now introduce the languages and the training datasets, explaining similarities and differences between training sets on the one hand and development and test sets on the other.
%In this subsection we shortly introduce the languages, the training datasets and the differences between them and the evaluation sets. %development and test sets.   

\paragraph{Spanish--Wixarika}
Wixarika (also known as Huichol) with ISO code \texttt{hch} is spoken in Mexico and belongs to the Yuto-Aztecan linguistic family. The training, development and test sets all belong to the same dialectal variation, Wixarika of Zoquipan, and use the same orthography. However, word boundaries are not always marked according to the same criteria in development/test and train. The training data \cite{mager2018probabilistic} is a translation of the fairy tales of Hans Christian Andersen and contains word acquisitions and
code-switching.

\paragraph{Spanish--Nahuatl}
Nahuatl is a Yuto-Aztecan language spoken in Mexico and El Salvador, with a wide dialectal variation (around 30 variants). For each main dialect a specific ISO 639-3 code is available.\footnote{
ISO 639-3 for the Nahutal languages: \texttt{
nci,  nhn,  nch,  ncx,  naz,  nln,  nhe,  ngu,  azz,  nhq,  nhk,  nhx,  nhp,  ncl,  nhm,  nhy,  ncj,  nht,  nlv,  ppl,  nhz,  npl,  nhc,  nhv,  nhi,  nhg,  nuz,  nhw,  nsu,  xpo,  nhn,  nch,  ncx,  naz,  nln,  nhe,  ngu,  azz,  nhq,  nhk,  nhx,  nhp,  ncl,  nhm,  nhy,  ncj,  nht,  nlv,  ppl,  nhz,  npl,  nhc,  nhv,  nhi,  nhg,  nuz,  nhw,  nsu,} and \texttt{xpo}. 
} %TODO: see how to add codes 
There is a lack of consensus regarding the orthographic standard.  This is very noticeable in the training data: the train corpus \cite{gutierrez-vasques-etal-2016-axolotl} has dialectal, domain, orthographic and diachronic variation (Nahuatl side). However, the majority of entries are closer to a Classical Nahuatl orthographic ``standard''.

The development and test datasets were translated to modern Nahuatl. In particular, the translations belong to Nahuatl Central/Nahuatl de la Huasteca (Hidalgo y San Luis Potosí) dialects. In order to be closer to the training corpus, an orthographic normalization was applied. %Therefore, these texts are also closer to Classical Nahuatl orthography. 
A simple  rule based  approach was used, which was based on the most predictable orthographic changes between modern varieties  and Classical Nahuatl.

\paragraph{Spanish–-Guarani}
Guarani is mostly spoken in Paraguay, Bolivia, Argentina and Brazil. It belongs to the Tupian language family (ISO \texttt{gnw, gun, gug, gui, grn, nhd}).  
The training corpus for Guarani \cite{chiruzzo-etal-2020-development} was collected from web sources (blogs and news articles) that contained a mix of dialects, from pure Guarani to more mixed Jopara %\manuel{Is that term correct? If yes, please explain} 
which combines Guarani with Spanish neologisms. %\manuel{Please add the variant of guarani of those texts}.
The development and test corpora, on the other hand, are in standard Paraguayan Guarani. %\manuel{Can you add the variant of the translaitons?}.


\paragraph{Spanish–-Bribri}

Bribri is a Chibchan language spoken in southern Costa Rica (ISO code \texttt{bzd}).
The training set for Bribri was extracted from six sources \cite{feldman-coto-solano-2020-neural,margery,gramaticacarla,cursobribri,cursoCarla,itte,corpusSofia}, including a dictionary, a grammar, two language learning textbooks, one storybook and the transcribed sentences from one spoken corpus. The sentences belong to three major dialects: Amubri, Coroma and Salitre. 

There are numerous sources of variation in the Bribri data \cite{feldman-coto-solano-2020-neural}: 1) There are several different orthographies, which use different diacritics for the same words. %(e.g. nasalization can be indicated with a line underneath the vowel, a tilde over the vowel or a Polish hook attached to the vowel).
2) The Unicode encoding of visually similar diacritics differs among authors.
3) There is phonetic and lexical variation across dialects. 4) There is considerable idiosyncratic variation between writers, including variation in word boundaries (e.g. \textit{ikíe} vrs \textit{i kie} "it is called"). In order to build a standardized training set, an intermediate orthography was used to make these different forms comparable and learning easier.
All of the training sentences are comparable in domain; they come from either traditional stories or language learning examples. Because of the nature of the texts, there is very little code-switching into Spanish. This is different from regular Bribri conversation, which would contain more borrowings from Spanish and more code-switching. The development and test sentences were translated by a speaker of the Amubri dialect and transformed into the intermediate orthography.


\paragraph{Spanish–-Rarámuri}
Rarámuri is a Uto-Aztecan language, spoken in northern Mexico (ISO: \texttt{tac, twr, tar, tcu, thh}). Training data for Rarámuri consists of a set of extracted phrases from the Rarámuri dictionary \citet{brambila1976diccionario}. However, we could not find any description of the dialectal variation to which these examples belong. The development and test set are translations from Spanish into the highlands Rarámuri variant (\texttt{tar}), and may differ from the training set. As with many polysynthetic languages, challenges can arise when the boundaries of a morpheme and a word are not clear and have no consensus. Native speakers, even with a standard orthography and from the same dialectal variation, may define words in a different standards to define word boundaries.

\paragraph{Spanish–-Quechua}
Quechua is a family of languages spoken in Argentina, Bolivia, Colombia, Ecuador, Peru, and Chile with many ISO codes for its language (\texttt{quh, cqu, qvn, qvc, qur, quy, quk, qvo, qve}, and  \texttt{quf}).
The development and test sets are translated into the standard version of Southern Quechua, specifically the Quechua Chanka (Ayacucho, code: \texttt{quy}) variety. This variety is spoken in different regions of Peru, and it can be understood in different areas of other countries, such as Bolivia or Argentina. This is the variant used on Wikipedia Quechua pages, and by Microsoft in its translations of software into Quechua. Southern Quechua includes different Quechua variants, such as Quechua Cuzco (\texttt{quz}) and Quechua Ayacucho (\texttt{quy}). %We provided training datasets for both variants: JW300 \cite{agic2019jw300} (\texttt{quy}, \text{quz}): Jehova's Witnesses texts, available in OPUS. We are also providing the parallel data aligned with English as an extra. MINEDU (\texttt{quy}): Sentences extracted from the official dictionary of the Minister of Education (MINEDU) in Peru for Quechua Ayacucho. Dict misc (quy): Dictionary entries and samples collected and reviewed.
Training datasets are provided for both variants. These datasets were created from JW300 \cite{agic-vulic-2019-jw300}, which consists of Jehovah's Witness texts, sentences extracted from the official dictionary of the Minister of Education (MINEDU), and miscellaneous dictionary entries and samples which have been collected and reviewed by \citet{Taquiri2020}.

%In the process of translating the development and test sets, the handling of pentavocalism from other regions, such as Collao Quechua and the apostrophe, is not used in Quechua Chanka. But normally both varieties are understood, since they share interculturality. In the suffixes there will be some limitations. Example in Quechua of variety chanka, kachkanchik will end with K while in Quechua of variety Collao it ends with S as for example Kachkanchis.

%There are different varieties of Quechua, they are Quechua Chanka, Quechua Collao, Quechua Wanka and Central Quechua. This language of variety Chanka and Collao share the lexicon, although Quechua Collao handles pantavocalism and Chanka trivocavolismo are understood correctly, while Central Quechua moves away. It is worth mentioning that these two varieties are the most widely spoken.


\paragraph{Spanish--Aymara}
Aymara is a Aymaran language spoken in Bolivia, Peru, and Chile (ISO codes \texttt{aym, ayr, ayc}).
The development and test sets are translated into the Central Aymara variant (\texttt{ayr}), specifically Aymara La Paz jilata, the largest variant. This is similar to the variant of the available training set, which is obtained from Global Voices \cite{prokopidis-etal-2016-parallel} (and published in OPUS \cite{tiedemann-2012-parallel}), a news portal translated by volunteers. However, the text may have potentially different writing styles that are not necessarily edited.

%There are many variants in Aymara. The Aymara of Pacajes is different from Los Andes, Omasuyos, Camacho, Franz Tamayo, etc. Though there may be variations in some terminologies or even grammar, all or most Aymara dialects are mutually intelligible.

%To leave for example: Sarxma, sarawayxä, sarxä, etc.
%Kid for example: wawa, yaya, yuqallwawa, lala, etc.


\paragraph{Spanish-–Shipibo-Konibo}
Shipibo-Konibo is a Panoan language spoken in  Perú (ISO \texttt{shp} and \texttt{kaq}).
The training sets for Shipibo-Konibo have been obtained from different sources and translators: Sources include translations of a sample from the Tatoeba dataset \cite{montoya-etal-2019-continuous}, translated sentences from books for bilingual education \cite{galarreta-etal-2017-corpus}, and dictionary entries and examples \cite{Loriot1993DiccionarioS}. 
%i) Flashcards, A sample from the Tatoeba dataset translated into Shipibo-Konibo; ii) Educational, Translated sentences from books for bilingual education; iii) and Dictionary: SIL dictionary entries and examples.
%\manuel{Are there citation available for this sources?} 
Translated text was created by a bilingual teacher, and follows the most recent guidelines of the Minister of Education in Peru, however, the third source is an extraction of parallel sentences from an old dictionary. %\manuel{Please add the dialect and writing system used for test and dev sets.} 
The development and test sets were created following the official convention as in the translated training sets. 

\paragraph{Spanish–-Asháninka}
Asháninka is an Arawakan language (ISO: \texttt{cni}) spoken in Peru and Brazil. Training data was created by collecting texts from different domains such as traditional stories, educational texts, and environmental laws for the Amazonian region \cite{ortega-etal-2020-overcoming,romano2008dic,mihas2011idioma}. 
%  Three things are important to know about the texts that are included in the training data 
The texts belong to domains such as: traditional stories, educational texts, environmental laws for the Amazonian region.
Not all the texts are translated into Spanish, there is a small fraction of these that are translated into Portuguese because a dialect of pan-Ashaninka is also spoken in the state of Acre in Brazil.
The texts come from different pan-Ashaninka dialects and have been normalized using the AshMorph \cite{ortega-etal-2020-overcoming}.
%\manuel{Check if it is ok to put this information back}
There are many neologisms that are not spread to the speakers of different communities. %\manuel{Is the dev/train sets in the same dialect/s as training?}. 
The translator of the development and test sets only translated the words and concepts that are well known in the communities, whereas other terms are preserved in Spanish. Moreover, the development and test sets were created following the official writing convention proposed by the Peruvian Government and taught in bilingual schools.

%%%%%%%%%%%%% New Proposed Teams Table %%%%%%%%%%%%%
% \begin{table*}[h]
%     \centering
%     % \setlength{\tabcolsep}{4.5pt}
%     \begin{adjustbox}{width=\textwidth}
%     \begin{tabular}{lcccccccccc}
%         \toprule
%         \multirow{1}{*}{\bf Team} & \multirow{1}{*}{\bf Langs.} & \multirow{1}{*}{\bf Sub.} & \multicolumn{5}{c}{\textbf{Data Sources}} &\multirow{1}{*}{\bf Arch.} &\multirow{1}{*}{\bf Multilingual} &\multirow{1}{*}{\bf Pretrained} \\
%         &&&Bible & JW300 & Wiki & Other Ext. & No Add. &&&\\
%         \midrule
        
%         CoAStaL &  10 & 20 & \checkmark & \checkmark & \checkmark & & & SMT & & \\
%         Helsinki & 10 & 50 & \checkmark &           &               & \checkmark & & Transf. & & \checkmark  \\
%         NRC-CNRC & 4 & 17 &&&&&\checkmark & Transf. & \checkmark &  \\
%         REPUcs & 1 & 2 & & \checkmark &&&& Transf. & \checkmark & \checkmark \\
%         Tamalli & 10 & 42 &&&&&& SMT; Transf. & \checkmark & \\
%         UBC-NLP & 8 & 29 & \checkmark & & \checkmark &&& T5 & \checkmark & \checkmark \\
%         UTokyo & 10 & 40 &&&&\checkmark&& mBART & \checkmark & \checkmark \\
%         Anonymous & 8 & 14 \\

%         \bottomrule
%     \end{tabular}
%     \end{adjustbox}
%     \caption{Participating teams (\emph{Team}) with system description paper. The information contained in this table is as follows:  number of languages that submissions  were submitted (\emph{Langs.}), total number of submission (\textit{Sub.}), a brief summary of external (Ext.) data sources used or \textit{No Add.} if no external data was used, system architecture, usage of a multilingual model (\emph{Multilingual}), and the usage of pretraining (\emph{Pretrained}). For more details we refer to the system description paper of each system.}
%     \label{tab:teams}
% \end{table*}
%%%%%%%%%%%%% End Proposed Teams Table %%%%%%%%%%%%%%%%%



\begin{table*}[h]
    \centering
    \setlength{\tabcolsep}{5pt}
    \small
    \begin{tabular}{p{0.16\textwidth} c c p{0.18\textwidth} p{0.13\textwidth} p{0.13\textwidth} p{0.13\textwidth}}
        \toprule
        \bf Team & \bf Langs. & \bf Sub. & \bf Data & \bf Models & \bf Multilingual & \bf Pretrained \\\midrule
        
        \Coastal~ \cite{bollman-etal-2021-moses}&  10 & 20 & Bible, JW300, OPUS, Wikipedia, New collected data & PB-SMT, Constrained Random Strings & No & No\\
        
        \Helsinki~ \cite{vazquez-etal-2021-helsinki}&  10 & 50 & Bible, OPUS, Constitutions, Normalization, Filtering, Back-Translation& Transformer NMT & Yes, all ST languages + Spanish-English & No\\
        
        \NRC~ \cite{knowles-etal-2021-nrc} & 4 & 17 & No external data, preoricessing, BPE Dropout.  & Transofrmer NMT & Yes, 4-languages & No \\ 
        \REPUcs~ \cite{moreno-2021-repu}&  1 & 2 & JW300, New dataset, Europarl & Transformer NMT. & Yes, with Spanish-English & Spanish-English pretraining\\
        
        \Tamalli~ \cite{parida-etal-2021-open}&  10 & 42 & - & WB-SMT. Transformer NMT, & 10-languages & No\\
        
        \UBC~ \cite{Billah-etal-2021-indt5}& 8 & 29 & Bible, Wikipedia & Transformer T5 & 10-Languages & New T5\\
        
        \UTokyo~\cite{zheng-etal-2021-low}& 10 & 40 & Monolingual from other languages. Data& Transformer & Yes & New mBART\\
        Anonymous & 8 & 14 & - & - & - & - \\
        \bottomrule
    \end{tabular}
    \caption{Participating team (\emph{Team}) with system description paper, number of languages that system outputs  were submitted for (\emph{Langs.}), total number of submissions (\textit{Sub.}), external data (\emph{Data}), models (\emph{Models}), 
    if training was multilingual (\emph{Multilingual}), and if pretraining was done (\emph{Pretrained}). More details can be found in the text.}
    \label{tab:teams}
\end{table*}

\paragraph{Spanish-–Otomí}
Otomí (also known as Hñähñu, Hñähño, Ñhato, Ñûhmû, depending on the region) is an Oto-Manguean language spoken in Mexico (ISO codes: \texttt{ott, otn, otx, ote, otq, otz, otl, ots, otm}). The training set\footnote{Otomí online corpus: https://tsunkua.elotl.mx/about/} was collected from a set of different sources, which implies that the text contains more than one dialectal variation and orthographic standard, however, most texts belong to the Valle del Mezquital  dialect (\texttt{ote}). This was specially challenging for the translation task, since the development and test sets are from the Ñûhmû de Ixtenco, Tlaxcala, variant (\texttt{otz}), which also has its own orthographic system. This variant is especially endangered as less than 100 elders still speak it. 



\subsection{External Data Used by Participants}
\label{subsec:additional_datasets}
In addition to the provided datasets, participants also used additional publicly available parallel data, monolingual corpora or newly collected data sets. The most common datasets were JW300 \cite{agic-vulic-2019-jw300} and the Bible's New Testament \cite{mayer2014creating,christodouloupoulos2015massively,mccarthy-etal-2020-johns}. Besides those, GlobalVoices \cite{prokopidis-etal-2016-parallel} and datasets available at OPUS \cite{tiedemann-2012-parallel} were added. New datasets were extracted from constitutions, dictionaries, and educational books. For monolingual text,  Wikipedia was most commonly used, assuming one was available in a language.


\section{Baseline and Submitted Systems}
\label{sec:systems}
%System's descriptions
We will now describe our baseline as well as all submitted systems. An overview of all teams and the main ideas going into their submissions is shown in Table \ref{tab:teams}.

\subsection{Baseline}
\label{subsec:baseline}

Our baseline system was a transformer-based sequence to sequence model \cite{vaswani-etal-2017}. We employed the hyperparameters proposed by \citet{guzman-etal-2019-flores} for a low-resource scenario. We implemented the model using Fairseq \cite{ott2019fairseq}. The implementation of the baseline can be found in the official shared task repository.\footnote{ \url{https://github.com/AmericasNLP/americasnlp2021}}

\subsection{University of British Columbia}

The team of the University of British Columbia  \citep[\UBC;][]{Billah-etal-2021-indt5} participated for all ten language pairs and in both tracks. They used an encoder-decoder transformer model based on T5 \cite{raffel2020exploring}. This model was pretrained on a dataset consisting of 10 indigenous languages and Spanish, that was collected by the team from different sources such as the Bible and Wikipedia, totaling 1.17 GB of text. However, given that some of the languages have more available data than others, this dataset is unbalanced in favor of languages like Nahuatl, Guarani, and Quechua. The team also proposed a two-stage fine-tuning method: first fine-tuning on the entire dataset, and then only on the target languages. %The model and collected data were made publicly available. 

\subsection{Helsinki}
The University of Helsinki \citep[\Helsinki;][]{vazquez-etal-2021-helsinki} participated for all ten language pairs in both tracks. This team did an extensive exploration of the existing datasets, and collected additional resources both from commonly used sources such as the Bible and Wikipedia, as well as other minor sources such as constitutions. Monolingual data was used to generate paired sentences through back-translation, and these parallel examples were added to the existing dataset. Then, a normalization process was done using existing tools, and the aligned data was further filtered. The quality of the data was also considered, and each dataset was assigned a weight depending on a noisiness estimation. The team used a transformer sequence-to-sequence model trained via two steps. For their main submission they first trained on data which was 90\% Spanish--English and 10\% indigenous languages, and then changed the data proportion to 50\% Spanish--English and 50\% indigenous languages. %To implement the described system the OpenNMT-py \cite{klein-etal-2017-opennmt} toolkit was used. 
%This system achieved best results for all language pairs in Track 1 as well as for 9 out of 10 in Track 2.

\subsection{CoAStaL}
The team of the University of Copenhagen (\Coastal) submitted systems for both tracks \cite{bollman-etal-2021-moses}. They focused on additional data collection and tried to improve the results with low-resource techniques. The team discovered that it was even hard to generate correct words in the output and that phrase-based statistical machine translation (PB-SMT) systems work %surprisingly 
well when compared to the state-of-the-art neural models. %\gn{I don't know if this is \emph{that} surprising, given that PB-SMT models have often been reported to do well when little data is available \citep{koehn-knowles-2017-six}. Maybe this statement could be toned down here and in the following section?}\manuel{Done} 
Interestingly, the team introduced a baseline that mimicked the target language using a character-trigram distribution and length constraints without any knowledge of the source sentence. This random text generation achieved even better results than some of the other submitted systems. The team also reported failed experiments, where character-based neural machine translation (NMT), pretrained transformers, language model priors, and graph convolution encoders using UD annotations could not get any meaningful results. 

\subsection{REPUcs}

The system of the Pontificia Universidad Cat\'olica del Per\'u \cite[\REPUcs;][]{moreno-2021-repu} submitted to the 
the Spanish--Quechua language pair in both tracks. The team collected external data from 3 different sources and analyzed the domain disparity between this training data and the development set. To solve the problem of domain mismatch, they decided to collect additional data that could be a better match for the target domain. The used data from a handbook \cite{iter-ortiz-2019-Runasimita}, a lexicon,\footnote{\url{https://www.inkatour.com/dico/}} and poems on the web \cite{duran2010lengua}.\footnote{  \url{https://lyricstranslate.com/}} Their model is a transformer encoder-decoder architecture with SentencePiece \cite{kudo-richardson-2018-sentencepiece} tokenization. Together with the existing parallel corpora, the new paired data was used for finetuning on top of a pretrained Spanish--English translation model. The team submitted two versions of their system: the first was only finetuned on JW300+ data, while the second one additionally leveraged the newly collected dataset. 
%The best result of both versions was the one that had the new dataset, achieven the best results for Spanish--Quechua on track 2 (see \S\ref{sec:Results}).
\begin{table*}
\centering
\makebox[0pt][c]{\parbox{1.2\textwidth}{%
    \begin{minipage}[b]{0.45\hsize}\centering
        \setlength{\tabcolsep}{4.5pt}
    \small
    \begin{tabular}{c c c r| r r}
Lang. &Rank	&Team	&Sub	&BLEU	&ChrF \\\hline
\multirow{8}{*}{aym}&1	&Helsinki &	2	&2.80	&\bf 31.0\\
&2	&Helsinki &	1	&2.91	&30.2\\
&3	&Helsinki &	3	&2.35	&26.1\\
&4	&UTokyo   & 1   &1.17   &21.4\\
&5	&CoAStaL &	1	&1.11	&19.1\\
&6	&UBC-NLP &	2	&0.99	&19.0\\
&7	&UBC-NLP & 	4	&0.76	&18.6\\
&8	&UTokyo&	2 &	1.18	&14.9\\
&9	&Anonym& 1 &	0.01	& 7.3\\\hline
&Rank	&Team	&Sub	&BLEU	&ChrF\\\hline
\multirow{9}{*}{bzd}&1	&Helsinki	&2	&5.18	&\bf 21.3\\
&2	&Helsinki	&1	&4.93	&20.4\\
&3	&CoAStaL	&1	&3.60	&19.6\\
&4	&Helsinki	&3	&3.68	&17.7\\
&5	&UTokyo	&1	&1.70	&14.3\\
&6	&UBC-NLP	&2	&0.94	&11.3\\
&7	&UTokyo	&2	&1.28	&11.2\\
&8	&UBC-NLP	&4	&0.89	&11.1\\
&9	&Anonym	&1	&0.14	&6.1\\\hline
Lang. &Rank	&Team	&Sub	&BLEU	&ChrF \\\hline
\multirow{9}{*}{cni}&1	&Helsinki	&2	&6.09	&\bf 33.2 \\
&2	&Helsinki	&1	&5.87	&32.4 \\
&3	&Helsinki	&3	&5.00	&30.6 \\ 
&4	&CoAStaL	&1	&3.02	&26.5 \\
&5	&UTokyo	&1	&0.20	&21.6 \\
&6	&UTokyo	&2	&0.84	&18.9 \\
&7	&UBC-NLP	&2	&0.08	&18.3 \\
&8	&UBC-NLP	&4	&0.09	&17.8 \\
&9	&Anonym	&1	&0.08	&11.4 \\\hline
Lang.&Rank	&Team	&Sub	&BLEU	&ChrF \\\hline
\multirow{11}{*}{gn}&1	&Helsinki	&2	&8.92	&\bf 37.6 \\
&2	&Helsinki	&1	&8.18	&36.7 \\
&3	&Helsinki	&3	&5.97	&31.1 \\
&4	&NRC-CNRC	&0	&4.73	&30.4 \\
&5	&NRC-CNRC	&4	&5.27	&30.3 \\
&6	&NRC-CNRC	&2	&4.06	&28.8 \\
&7	&UTokyo	&1	&3.21	&26.5 \\
&8	&CoAStaL	&1	&2.20	&24.1 \\
&9	&UTokyo	&2	&3.18	&23.3 \\
&10	&NRC-CNRC	&3	&0.64	&16.3 \\
&11	&Anonym	&1	&0.03	&8.5 \\\hline
Lang &Rank	&Team	&Sub	&BLEU	&ChrF \\\hline
\multirow{12}{*}{hch}&1	&Helsinki	&2	&15.67	&\bf 36.0\\
&2	&Helsinki	&1	&14.71	&34.8\\
&3	&NRC-CNRC	&0	&14.90	&32.7\\
&4	&NRC-CNRC	&2	&13.65	&31.5\\
&5	&Helsinki	&3	&13.72	&31.1\\
&6	&CoAStaL	&1	&8.80	&25.7\\
&7	&UTokyo	&1	&7.09	&23.8\\
&8	&NRC-CNRC	&3	&4.62	&20.0\\
&9	&UBC-NLP	&2	&5.52	&19.5\\
&10	&UBC-NLP	&4	&5.09	&18.6\\
&11	&UTokyo	&2	&6.30	&18.4\\
&12	&Amonym	&1	&0.06	&8.1\\
        \end{tabular}
    \end{minipage}
    \begin{minipage}[b]{0.45\hsize}\centering
        \setlength{\tabcolsep}{4.5pt}
    \small
    \begin{tabular}{c c c r| r r}
Lang &Rank	&Team	&Sub	&BLEU	&ChrF \\\hline
\multirow{12}{*}{nah}&1	&Helsinki	&2	&3.25	&\bf 30.1 \\
&2	&Helsinki	&1	&2.8	&29.4 \\
&3	&NRC-CNRC	&0	&2.13	&27.7 \\
&4	&NRC-CNRC	&2	&1.78	&27.3 \\
&5	&Helsinki	&3	&2.76	&27.3 \\
&6	&UTokyo	&1	&0.55	&23.9 \\
&7	&CoAStaL	&1	&2.06	&21.4 \\
&8	&UTokyo	&2	&0.98	&19.8 \\
&9	&UBC-NLP	&2	&0.16	&19.6 \\
&10	&NRC-CNRC	&3	&0.14	&18.1 \\
&11	&Anonym	&2	&0.09	&10.3 \\
&12	&Anonym	&3	&0.09	&9.7 \\
&13	&Anonym	&4	&0.08	&9.5 \\
&14	&Anonym	&1	&0.04	&8.7 \\\hline
Lang &Rank	&Team	&Sub	&BLEU	&ChrF \\\hline
\multirow{12}{*}{oto}&1	&Helsinki	&2	&5.59	&\bf 22.8 \\
&2	&Helsinki	&1	&3.85	&19.1 \\
&3	&CoAStaL	&1	&2.72	&18.4 \\
&4	&Helsinki	&3	&2.9	&18.1 \\
&5	&UTokyo	&2	&2.45	&15.2 \\
&6	&UTokyo	&1	&0.12	&12.8 \\
&7	&Anonym&1	&0.15	&10.2 \\
&8	&UBC-NLP	&2	&0.04	&8.4 \\
&9	&UBC-NLP	&4	&0.04	&8.3 \\\hline
Lang &Rank	&Team	&Sub	&BLEU	&ChrF \\\hline
\multirow{12}{*}{quy}&1	&Helsinki	&2	&5.38	&\bf 39.4 \\
&2	&Helsinki	&1	&5.16	&38.3 \\
&3	&REPUcs	&2	&3.1	&35.8 \\
&4	&UTokyo	&1	&2.35	&33.2 \\
&5	&UTokyo	&2	&2.62	&32.8 \\
&6	&Helsinki	&3	&3.56	&31.8 \\
&7	&CoAStaL	&1	&1.63	&26.9 \\
&8	&Anonym&2	&0.23	&10.3 \\
&9	&Anonym&4	&0.13	&9.8 \\
&10	&Anonym&1	&0.06	&9.0 \\
&11	&Anonym&3	&0.03	&6.6 \\\hline
Lang &Rank	&Team	&Sub	&BLEU	&ChrF \\\hline
\multirow{6}{*}{shp}&1	&Helsinki	&2	&10.49	&\bf 39.9 \\
&2	&Helsinki	&1	&9.06	&38.0 \\
&3	&CoAStaL	&1	&3.9	&29.7 \\
&4	&Helsinki	&3	&6.76	&28.6 \\
&5	&UTokyo	&1	&0.33	&16.3 \\
&6	&UTokyo	&2	&0.46	&15.5 \\
&7	&UBC-NLP	&2	&0.23	&12.4 \\\hline
Lang &Rank	&Team	&Sub	&BLEU	&ChrF \\\hline
\multirow{12}{*}{tar}&1	&Helsinki	&2	&3.56	&\bf 25.8 \\
&2	&Helsinki	&1	&3.24	&24.8 \\
&3	&NRC-CNRC	&0	&2.69	&24.7 \\
&4	&NRC-CNRC	&2	&2.1	&23.9 \\
&5	&Helsinki	&3	&1.8	&21.6 \\
&6	&NRC-CNRC	&3	&0.83	&16.5 \\
&7	&CoAStaL	&1	&1.05	&15.9 \\
&8	&UTokyo	&1	&0.1	&12.2 \\
&9	&UBC-NLP	&2	&0.05	&10.5 \\
&10	&UBC-NLP	&4	&0.1	&10.5 \\
&11	&UTokyo	&2	&0.69	&8.4
        \end{tabular}
    \end{minipage}
    \hfill
}}       
\caption{Results of Track 1 (development set used for training) for all systems and language pairs. The results are ranked by the official metric of the shared task: ChrF. One team decided to send a anonymous submission  (\textit{Anonym}). Best results are shown in bold, and they are significantly better than the second place team (in each language-pair) according to the Wilcoxon signed-ranked test and Pitman's permutation test with p$<$0.05 \cite{dror-etal-2018-hitchhikers}.}
\label{tab:track1}
\end{table*}
\subsection{UTokyo}

The team of the University of Tokyo  \citep[\texttt{UTokyo};][]{zheng-etal-2021-low} submitted systems for all languages and both tracks.
A multilingual pretrained encoder-decoder  model \citep[mBART;][]{liu-etal-2020-multilingual} was used, implemented with the Fairseq toolkit \cite{ott2019fairseq}. The model was first pretrained on a huge amount of data (up to 13GB) from various high-resource languages, and then finetuned for each target language using the official provided data.

\begin{table*}[]
    %\tiny
    \centering
    \setlength{\tabcolsep}{5.5pt}
    \small
    %\begin{adjustbox}{width=\columnwidth}
    %\resizebox{0.7\linewidth}{!}{%
    \begin{tabular}{l|cccccccccc|c}
        \toprule
        \textbf{System} &\textbf{aym} & \textbf{bzd} & \textbf{cni} & \textbf{gn} & \textbf{hch} & \textbf{nah} & \textbf{oto} & \textbf{quy} & \textbf{shp} & \textbf{tar} & \textbf{Avg.} \\
        \midrule
        Baseline & {49.33} & \textbf{52.00} & {42.80} & {55.87} & {41.07} & {54.07} & 36.50 & 59.87 & {52.00} & {43.73} &{48.72} \\
        Helsinki-5 & \textbf{57.60} & 48.93 & \textbf{55.33} & \textbf{62.40} & \textbf{55.33} & \textbf{62.33} & \textbf{49.33} & \textbf{60.80} & \textbf{65.07} & \textbf{58.80} & 57.59 \\
        NRC-CNRC-1 & - & - & - & 57.20 & 50.40 & 58.94 & - & - & - & 53.47 & 55.00$^*$ \\
        %final
    \bottomrule
    \end{tabular}
    %}
    %\end{adjustbox}
    \caption{Results of the NLI analysis. * indicates that the average score is not directly comparable as the number of languages differs for the given system.%\gn{There are 4 significant digits here, are the test sets large enough to support this level of precision in result reporting?}\gn{What do bold numbers indicate (here and elsewhere)? Did you do significance tests to measure the significance of the results?}
    }
    \label{tab:nli_analysis}
\end{table*}

\subsection{NRC-CNRC}

The team of the National Research Council Canada \citep[\NRC;][]{knowles-etal-2021-nrc} submitted systems for the Spanish to Wixárika, Nahuatl, Rarámuri and Guarani language pairs for both tracks. 
Due to ethical considerations, the team decided not to use external data, and restricted themselves to the data provided for the shared task. All data was preprocessed with standard Moses tools \cite{koehn2007moses}. The submitted systems were based on a Transformer model, and used BPE for tokenization. The team experimented with multilingual models pretrained on either 3 or 4 languages, finding that the 4 language model achieved higher performance. Additionally the team trained a Translation Memory \cite{simard2012poor} using half of the examples of the development set. Surprisingly, even given its small amount of training data, this system outperformed the team's Track 2 submission for Rarámuri.


% The system used for submission was based on a Transformer model and used BPE for tokenization, using the Sockeye framework \cite{hieber-etal-2020-sockeye}, using a multilingual model pretrained on data from all 4 languages languages and a small version of only 3 languages. Additionally, the team investigated the effect of BPE-dropout \cite{sennrich2016edinburgh} and obtained mixed results. This model was later finetuned to each of the language pairs. For Track 1, the team used a part of the development set to finetune the systems, with the goal of achieving domain or dialect adaptation.   
% The team also performed a Translation Memory evaluation \cite{simard2012poor}. 

\subsection{Tamalli}

The team \texttt{Tamalli}\footnote{Participating universities: Idiap Research Institute, City University of New York, BITS-India, Universidad Autónoma Metropolitana-México, Ghent University, and Universidad Politécnica de Tulancingo-México } \cite{parida-etal-2021-open} participated in Track 1 for all 10 language pairs. 
%It achieved the second highest score for 3 languages  
The team used an IBM Model 2 for SMT, and a transformer model for NMT. The team's NMT models were trained in two settings: one-to-one, with one model being trained per target language, and one-to-many, where decoder weights were shared across languages and a language embedding layer was added to the decoder. They submitted 5 systems per language, which differed in their hyperparameter choices and training setup. 
%The SMT model achieved the best performance for 6/10 languages, and a one-to-one transformer achieved the best performance for 2/10 languages. Of the three languages for which the team achieved the second highest score, 2 were achieved by the statistical model.


\section{Results}
\label{sec:Results}
%In this section we present the results of the AmericasNLP shared task for open machine translation. For all language pairs and system, we observe extremely low automatic scores likely due to the low amounts of available data, with an additional mismatch of domain, dialect and orthography between the evaluation sets and the training sets \cite{knowles-etal-2021-nrc}.  
\subsection{Track 1}
\label{subsub:results_t1}

The complete results for all systems submitted to Track 1 are shown in Table \ref{tab:track1}. 
Submission 2 of the \Helsinki~ team achieved first place for all language pairs. 
%System 2 follows a strategy of multilingual machine translation in two steps, with a first step training mostly on the English--Spanish set (90\%), and then decreasing this ratio afterward to 50\%. Also, in submission 2, the team used 100\% of the development for the training set for the final model. Together with text normalization among datasets and back translation for monolingual indigenous text, this strategy showed a huge improvement. 
Interestingly, for all language pairs, the \Helsinki~ team also achieved the second best result with their Submission 1. Submission 3 was less successful, achieving third place on three pairs.
The \NRC~ team achieved third place for Wixárika, Nahuatl, and Rarámuri, and fourth for Guarani.%, which were all the language pairs they participated in, demonstrating the advantages of using a multilingual model. 
The lower automatic scores of their systems can also be partly due to the team not using additional datasets. The \REPUcs~ system obtained the third best result for Quechua, the only language they participated in. \Coastal's first system, a PB-SMT model, achieved third place for Bribri, Otomí, and Shipibo-Konibo, and fourth place for Ashaninka. This suggests that SMT is still competitive for low-resource languages. \UTokyo~ and \UBC~ 
%chose the strategy of using pretrained models. \UToyko~ used an mBART pretrained model, while \UBC~ decided to train a T5-style model with a custom collected dataset. Both approaches 
were less successful than the other approaches. Finally, we attribute the bad performance of the anonymous submission to a possible bug. Since our baseline system was not trained on the development set, no specific baseline was available for this track.

%Helsinki won. better luck next year! :D


\begin{table*}
\centering
\makebox[0pt][c]{\parbox{1.2\textwidth}{%
    \begin{minipage}[b]{0.45\hsize}\centering
        \setlength{\tabcolsep}{4.5pt}
    \small
    \begin{tabular}{c c c r| r r}
Lang. &Rank	&Team	&Sub#	&BLEU	&ChrF \\\hline
\multirow{12}{*}{aym}&1	&Helsinki	&5	&2.29	&\bf 28.3 \\
&2	&Helsinki	&4	&1.41	&21.6 \\
&3	&UTokyo	&3	&1.03	&20.9 \\
&4	&Tamalli	&1	&0.03	&20.2 \\
&5	&Tamalli	&3	&0.39	&19.4 \\
&6	&UBC-NLP	&3	&0.82	&18.2 \\
&7	&UBC-NLP	&1	&1.01	&17.8 \\
&8	&UTokyo	4&	&1.34	&17.2 \\
&9	&CoAStaL	&2	&0.05	&16.8 \\
&10	&Tamalli	&2	&0.07	&16.6 \\
&11	&Baseline	&1	&0.01	&15.7 \\
&12	&Tamalli	&5	&0.12	&15.1 \\
Lang. &Rank	&Team	&Sub#	&BLEU	&ChrF \\\hline
\multirow{12}{*}{bzd}&1	&Helsinki	&5	&2.39	&\bf 16.5 \\
&2	&Tamalli	&3	&1.09	&13.2 \\
&3	&UTokyo	&3	&1.29	&13.1 \\
&4	&Helsinki	&4	&1.98	&13.0 \\
&5	&Tamalli	&1	&0.03	&11.3 \\
&6	&UBC-NLP	&1	&0.99	&11.2 \\
&7	&UBC-NLP	&3	&0.86	&11.0 \\
&8	&CoAStaL	&2	&0.06	&10.7 \\
&9	&Tamalli	&5	&0.36	&10.6 \\
&10	&UTokyo	&4	&1.13	&10.4 \\
&11	&Baseline	&1	&0.01	&6.8 \\
&12	&Tamalli	&2	&0.25	&3.7 \\
Lang. &Rank	&Team	&Sub#	&BLEU	&ChrF \\\hline
\multirow{12}{*}{cni}&1	&Helsinki	&5	&3.05	&\bf 25.8 \\
&2	&Tamalli	&1	&0.01	&25.3 \\
&3	&Helsinki	&4	&3.01	&23.6 \\
&4	&UTokyo	&3	&0.47	&21.4 \\
&5	&CoAStaL	&2	&0.03	&21.2 \\
&6	&Tamalli	&3	&0.18	&18.6 \\
&7	&UTokyo	&4	&0.76	&18.4 \\
&8	&UBC-NLP	&1	&0.07	&17.8 \\
&9	&UBC-NLP	&3	&0.09	&17.6 \\
&10	&Tamalli	&5	&0.07	&17.4 \\
&11	&Tamalli	&2	&0.06	&13.0 \\
&12	&Baseline	&1	&0.01	&10.2 \\
Lang. &Rank	&Team	&Sub#	&BLEU	&ChrF \\\hline
\multirow{12}{*}{gn}&1	&Helsinki	&5	&6.13	&\bf 33.6 \\
&2	&Helsinki	&4	&4.10	&27.6 \\
&3	&NRC-CNRC	&1	&2.86	&26.1 \\
&4	&UTokyo	&3	&3.16	&25.4 \\
&5	&UTokyo	&4	&2.97	&25.1 \\
&6	&Tamalli	&5	&1.90	&20.7 \\
&7	&Baseline	&1	&0.12	&19.3 \\
&8	&Tamalli	&3	&1.03	&18.7 \\
&9	&Tamalli	&1	&0.05	&17.2 \\
&10	&CoAStaL	&2	&0.03	&12.8 \\
&11	&Tamalli	&2	&0.13	&10.8 \\
Lang. &Rank	&Team	&Sub#	&BLEU	&ChrF \\\hline
\multirow{12}{*}{hch}&1	&Helsinki	&5	&9.63	&\bf 30.4 \\
&2	&NRC-CNRC	&1	&7.96	&26.4 \\
&3	&Helsinki	&4	&9.13	&25.4 \\
&4	&UTokyo	&3	&6.74	&22.9 \\
&5	&UTokyo	&4	&6.74	&21.6 \\
&6	&Tamalli	&1	&0.01	&21.4 \\
&7	&Tamalli	&3	&5.02	&20.6 \\
&8	&UBC-NLP	&1	&5.10	&19.4 \\
&9	&CoAStaL	&2	&2.07	&19.1 \\
&10	&UBC-NLP	&3	&4.95	&18.6 \\
&11	&Tamalli	&5	&4.71	&16.9 \\
&12	&Baseline	&1	&2.20	&12.6 \\
&13	&Tamalli	&2	&3.29	&9.4 \\
        \end{tabular}
    \end{minipage}
    \begin{minipage}[b]{0.45\hsize}\centering
        \setlength{\tabcolsep}{4.5pt}
    \small
    \begin{tabular}{c c c r| r r}
Lang &Rank	&Team	&Sub	&BLEU	&ChrF \\\hline
\multirow{12}{*}{nah}&1	&Helsinki	&5	&2.38	&\bf 26.6 \\
&2	&Helsinki	&4	&2.02	&24.3 \\
&3	&UTokyo	&4	&1.2	&23.8 \\
&4	&NRC-CNRC	&1	&0.83	&23.7 \\
&5	&UTokyo	&3	&0.29	&23.6 \\
&6	&Tamalli	&1	&0.03	&21.8 \\
&7	&UBC-NLP	&1	&0.12	&19.5 \\
&8	&UBC-NLP	&3	&0.15	&18.8 \\
&9	&CoAStaL	&2	&0.03	&18.4 \\
&10	&Tamalli	&3	&0.11	&17.4 \\
&11	&Tamalli	&5	&0.10	&16.6 \\
&12	&Baseline	&1	&0.01	&15.7 \\
&13	&Tamalli	&4	&0.08	&14.5 \\
&14	&Tamalli	&2	&0.03	&11.2 \\
Lang &Rank	&Team	&Sub	&BLEU	&ChrF \\\hline
\multirow{12}{*}{oto}&1	&Helsinki	&5	&1.69	&\bf 14.7 \\
&2	&Helsinki	&4	&1.37	&14.1 \\
&3	&UTokyo	&4	&1.28	&13.3 \\
&4	&UTokyo	&3	&0.05	&12.5 \\
&5	&Tamalli	&1	&0.01	&11.8 \\
&6	&Tamalli	&3	&0.12	&11.0 \\
&7	&CoAStaL	&2	&0.03	&10.1 \\
&8	&UBC-NLP	&1	&0.03	&8.2 \\
&9	&UBC-NLP	&3	&0.03	&8.1 \\
&10	&Tamalli	&5	&0.01	&7.4 \\
&11	&Baseline	&1	&0.00	&5.4 \\
&12	&Tamalli	&2	&0.00	&1.4 \\
Lang &Rank	&Team	&Sub	&BLEU	&ChrF \\\hline
\multirow{12}{*}{quy}&1	&REPUcs	&1	&2.91 & 34.6\\
&2	&Helsinki	&5	&3.63 & 34.3 \\
&3	&UTokyo	&4	&2.47 & 33.0\\
&4	&UTokyo	&3	&2.1 & 32.8\\
&5	&Baseline	&1	&0.05 & 30.4\\
&6	&Tamalli	&5	&0.96 & 27.3\\
&7	&Tamalli	&3	&0.64 & 26.3\\
&8	&Helsinki	&4	&2.67 & 25.2\\
&9	&Tamalli	&1	&0.22 & 24.4\\
&10	&Tamalli	&2	&0.69 & 23.2\\
&11	&CoAStaL	&2	&0.02 & 23.2\\
Lang &Rank	&Team	&Sub	&BLEU	&ChrF \\\hline
\multirow{12}{*}{shp}&1	&Helsinki	&5	&5.43	&\bf 32.9 \\
&2	&Helsinki	&4	&4.53	&29.4 \\
&3	&Tamalli	&1	&0.06	&20.4 \\
&4	&UTokyo	&3	&0.71	&17.5 \\
&5	&CoAStaL	&2	&0.04	&17.3 \\
&6	&UTokyo	&4	&0.64	&16.4 \\
&7	&Tamalli	&3	&0.31	&14.9 \\
&8	&Tamalli	&5	&0.28	&12.5 \\
&9	&UBC-NLP	&1	&0.16	&12.4 \\
&10	&Baseline	&1	&0.01	&12.1 \\
&11	&Tamalli	&2	&0.09	&8.9 \\
Lang &Rank	&Team	&Sub	&BLEU	&ChrF \\\hline
\multirow{12}{*}{tar}&1	&Helsinki	&5	&1.07	&\bf 18.4 \\
&2	&Tamalli	&1	&0.04	&15.5 \\
&3	&Helsinki	&4	&0.81	&15.5 \\
&4	&NRC-CNRC	&1	&0.27	&14.3 \\
&5	&UTokyo	&3	&0.06	&12.3 \\
&6	&UTokyo	&4	&0.06	&11.9 \\
&7	&CoAStaL	&2	&0.06	&11.3 \\
&8	&UBC-NLP	&1	&0.08	&10.2 \\
&9	&UBC-NLP	&3	&0.06	&10.2 \\
&10	&Tamalli	&4	&0.05	&8.9 \\
&11	&Tamalli	&3	&0.04	&8.4 \\
&12	&Tamalli	&5	&0.02	&7.3 \\
&13	&Baseline	&1	&0.00	&3.9 \\
&14	&Tamalli	&2	&0.01	&2.8 \\
        \end{tabular}
    \end{minipage}
    \hfill
}}       
\caption{Results of Track 2 (development set \emph{not} used for training) for all systems and language pairs. The results are ranked by the official metric of the shared task: ChrF. Best results per language pair are shown in bold, and they are significantly better than the second place team (in each language-pair) according to the Wilcoxon signed-ranked test and Pitman's permutation test with p$<$0.05 \cite{dror-etal-2018-hitchhikers}.}
\label{tab:track2}
\end{table*}


\subsection{Track 2}
\label{subsub:results_t2}
All results for Track 2, including those of our baseline system, are shown in Table \ref{tab:track2}. 

%Even with the low scores registered by all systems on automatic evaluation, 
Most submissions outperformed the baseline by a large margin. As for Track 1, the best system was from the \Helsinki~team (submission 5), winning  9 out of 10 language pairs. %Helsinki's submission 5 (Their best system) again performs a two-step training combined with English, and achieves better results than the pure multilingual approach. 
\REPUcs~ achieved the best score for Spanish--Quechua, the only language pair they submitted results for. Their pretraining on Spanish--English and the newly collected dataset proved to be successful. 

Second places were more diverse for Track 2 than for Track 1. The \NRC~ team achieved second place for two languages (Wixarika and Guarani), %out of four language pairs they submitted ; 
\UTokyo~achieved second place for three languages (Aymara, Nahuatl and Otomí), and the \Helsinki~team came in second for Quechua. \Tamalli~only participated in Track 2, with 4 systems per language. Their most successful one was submission 1, a word-based SMT system. 
%Similar to the findings for the SMT \Coastal system in Track 1.  
An interesting submission for this track was the \Coastal~submission 2, which created a random generated output that mimics the target language distribution. This system consistently outperformed the official baseline and even outperformed other approaches for most languages. 


\subsection{Supplementary Evaluation Results}


\begin{figure}[t!]
\begin{center}

\begin{subfigure}[t]{0.455\textwidth}
\caption{Shipibo-Konibo: Adequacy} 
\label{fig:shp}
\includegraphics[width=\linewidth,trim={0.5cm 0cm 0.5cm 1.6cm},clip]{figs/shp.stack.adequacy.pdf}
%\includegraphics[width=\linewidth,trim={0.5cm 0cm 0.5cm 1.6cm},clip]{figs/shp.pdf}
\end{subfigure}
\begin{subfigure}[t]{0.455\textwidth}
\caption{Otom\'i: Adequacy}
\label{fig:oto}
%\includegraphics[width=\linewidth,trim={0.5cm 0cm 0.5cm 1.6cm},clip]{figs/oto.pdf} 
\includegraphics[width=\linewidth,trim={0.5cm 0cm 0.5cm 1.6cm},clip]{figs/oto.stack.adequacy.pdf}
\end{subfigure}

\begin{subfigure}[t]{0.455\textwidth}
\caption{Shipibo-Konibo: Fluency} 
\label{fig:shp}
\includegraphics[width=\linewidth,trim={0.5cm 0cm 0.5cm 1.6cm},clip]{figs/shp.stack.fluency.pdf}
%\includegraphics[width=\linewidth,trim={0.5cm 0cm 0.5cm 1.6cm},clip]{figs/shp.pdf}
\end{subfigure}
\begin{subfigure}[t]{0.455\textwidth}
\caption{Otom\'i: Fluency}
\label{fig:oto}
%\includegraphics[width=\linewidth,trim={0.5cm 0cm 0.5cm 1.6cm},clip]{figs/oto.pdf} 
\includegraphics[width=\linewidth,trim={0.5cm 0cm 0.5cm 1.6cm},clip]{figs/oto.stack.fluency.pdf}
\end{subfigure}

\caption{Adequacy and fluency distribution scores for Shipibo-Konibo and Otom\'i. %\gn{I found these a bit hard to read, maybe stacked bar charts showing the proportion of each evaluation would be easier? \url{https://matplotlib.org/stable/gallery/lines_bars_and_markers/bar_stacked.html}}
}
\label{fig:boxplots}
\end{center}
\end{figure}


%\Manuel{Arturo, can you add here the scores and do some analysis? I can help too}
As explained in \S\ref{sec:task}, we also conducted a small human evaluation of system outputs based on adequacy and fluency on a 5-points scale, which was performed by a professional translator for two language-pairs: Spanish to Shipibo-Konibo and Otom\'i.\footnote{In the WMT campaigns, it is common to perform a crowd-sourced evaluation with several annotators. However, we cannot follow that procedure given the low chance to find native speakers of indigenous languages as users in crowd-sourcing platforms.} This evaluation was performed given the extremely low automatic evaluation scores, and the natural question about the usefulness of the outputs of MT systems at the current state-of-the-art. While we selected two languages as a sample to get a better approximation to this question, further studies are needed to draw stronger conclusions.


\begin{figure*}[t!]
\begin{center}

\begin{subfigure}[t]{0.475\textwidth}
\caption{Shipibo-Konibo: Adequacy} 
\label{fig:shp.ade}
\includegraphics[width=\linewidth,trim={0.75cm 0cm 0.75cm 1.2cm},clip]{figs/shp.chrf.adequacy.pdf}
\end{subfigure}
\begin{subfigure}[t]{0.475\textwidth}
\caption{Shipibo-Konibo: Fluency}
\label{fig:shp.flu}
\includegraphics[width=\linewidth,trim={0.75cm 0cm 0.75cm 1.2cm},clip]{figs/shp.chrf.fluency.pdf} 
\end{subfigure}

\begin{subfigure}[t]{0.475\textwidth}
\caption{Otom\'i: Adequacy} 
\label{fig:oto.ade}
\includegraphics[width=\linewidth,trim={0.75cm 0cm 0.75cm 1.6cm},clip]{figs/oto.chrf.adequacy.pdf}
\end{subfigure}
\begin{subfigure}[t]{0.475\textwidth}
\caption{Otom\'i: Fluency}
\label{fig:oto.flu}
\includegraphics[width=\linewidth,trim={0.75cm 0cm 0.75cm 1.6cm},clip]{figs/oto.chrf.fluency.pdf} 
\end{subfigure}

\caption{Relationship between ChrF scores and annotations for adequacy (left) and fluency (right).}
\label{fig:scatterplots}
\end{center}
\end{figure*}


Figure \ref{fig:boxplots} shows the adequacy and fluency scores annotated for Spanish--Shipibo-Konibo and Spanish--Otom\'i language-pairs.  %for the two target language-pairs, 
considering the baseline and the three highest ranked systems according to ChrF. For both languages, we observe that the adequacy scores are similar between all systems except for \Helsinki, the best ranked submission given the automatic evaluation metric, which has more variance than the others. However, the average score is low, around 2, which means that only few words or phrases express the meaning of the reference. 

Looking at fluency, there is less similarity between the Shipibo-Konibo and Otom\'i annotations. For Shipibo-Konibo, there is no clear difference between the systems in terms of their average scores. We note that \Tamalli's system obtained the larger group with the relatively highest score. For Otom\'i, the three submitted systems are at least slightly better than the baseline on average, but only in 1 level of the scale. The scores for fluency are similar to adequacy in this case. Besides, according to the annotations, the output translations in Shipibo-Konibo were closer to human-produced texts than in Otom\'i. %However, to confirm the insight, it would be preferred to have an extra annotator per language to study the inter-annotator agreement.

We also show the relationship between ChrF and the adequacy and fluency scores in Figure \ref{fig:scatterplots}. However, there does not seem to be a correlation between the automatic metric and the manually assigned scores. 

\subsection{Analysis: NLI}
One approach for zero-shot transfer learning of a sequence classification task is the translate-train approach, where a translation system is used to translate high-resource labeled training data into the target language. In the case of pretrained multilingual models, these machine translated examples are then used for finetuning. For our analysis, we used various shared task submissions to create different sets of translated training data. We then trained a natural language inference (NLI) model using this translated data, and used the downstream NLI performance as an extrinsic evaluation of translation quality. 

Our experimental setup was identical to \citet{ebrahimi2021americasnli}. We focused only on submissions from Track 2, and analyzed the \Helsinki-5 and the \NRC-1 system. We present results in Table \ref{tab:nli_analysis}. Performance from using the \Helsinki~ system far outperforms the baseline on average, and using the \NRC~ system also improves over the baseline. For the four languages covered by all systems, we can see that the ranking of NLI performance matches that of the automatic ChrF evaluation. Between the Helsinki and Baseline systems, this ranking also holds for every other language except for Bribri, where the Baseline achieves around 3 percentage points higher accuracy. Overall, this evaluation both confirms the ranking created by the ChrF scores and provides strong evidence supporting the use of translation-based approaches for zero-shot tasks.
%\gn{There are 4 significant digits here, are the test sets large enough to support this level of precision in result reporting?}\gn{What do bold numbers indicate (here and elsewhere)? Did you do significance tests to measure the significance of the results?}

% Complementary evaluation
% ...

\section{Error Analysis}
\label{sec:error_analysis}

To extend the analysis in the previous sections, Tables \ref{tab:shp-samples} and \ref{tab:oto-samples} show output samples using the best ranked system (\Helsinki-5) for Shipibo-Konibo and Otom\'i, respectively. In each table, we present the top-3 outputs ranked by ChrF and the top-3 ranked by Adequacy and Fluency.

For Shipibo-Konibo, in Table \ref{tab:shp-samples}, we observe that the first three outputs (with the highest ChrF) are quite close to the reference. Surprisingly, the adequacy annotation of the first sample is relatively low. We can also observe that many subwords are presented in both the reference and the system's output, but not entire words, which shows why BLEU may not be a useful metric to evaluate performance. However, the subwords are still located in different order, and concatenated with different morphemes, which impacts the fluency. Concerning the most adequate and fluent samples, we still observe a high presence of correct subwords in the output, and we can infer that the different order or concatenation of different morphemes did not affect the original meaning of the sentence.

For Otom\'i, in Table \ref{tab:oto-samples}, the scenario was less positive, as the ChrF scores are lower than for Shipibo-Konibo, on average. This was echoed in the top-3 outputs, which are very short and contain words or phrases that are preserved in Spanish for the reference translation. Concerning the most adequate and fluent outputs, we observed a very low overlapping of subwords (less than in Shipibo-Konibo), which could only indicate that the outputs preserve part of the meaning of the source but they are expressed differently than the reference. Moreover, we noticed some inconsistencies in the punctuation, which impacts in the ChrF overall score.

In summary, there are some elements to explore further in the rest of the outputs: How many loanwords or how much code-switched text from Spanish is presented in the reference translation? Is there consistency in the punctuation, e.g., period at the end of a segment, between all the source and reference sentences? %(e.g. end of sentence period). %or language-specific punctuation). 


\begin{table}[]
\setlength\tabcolsep{2.5pt}
\resizebox{\linewidth}{!}{%
\begin{tabular}{lp{9cm}}
Scores     & Sentences                     \\ \hline \hline
C: 66.7 & \textsc{\small src:} Un niño murió de los cinco.                  \\
A: 1       & \textsc{\small ref:} Westiora bakera mawata iki pichika batiayax. \\
F: 4       & \textsc{\small out:} Westiora bakera pichika mawata iki.      \\ \hline
C: 60.9 & \textsc{\small src:} Sé que no puedes oírme.                  \\
A: 4       & \textsc{\small ref:} Eanra onanke min ea ninkati atipanyama. \\
F: 3       & \textsc{\small out:} Minra ea ninkati atipanyamake.      \\ \hline
C: 60.1 & \textsc{\small src:} Necesito un minuto para recoger mis pensamientos.                  \\
A: 4       & \textsc{\small ref:} Eara westiora minuto kenai nokon shinanbo biti kopi. \\
F: 3       & \textsc{\small out:} Westiora serera ea kenai nokon shinanbo biti.      \\ \hline \hline

C: 57.1 & \textsc{\small src:} Hoy no he ido, así que no lo he visto.                   \\
A: 5       & \textsc{\small ref:} Ramara ea kama iki, jakopira en oinama iki. \\
F: 5       & \textsc{\small out:} Ramara ea kayamake, jaskarakopira en oinyamake      \\ \hline
C: 53.6 & \textsc{\small src:}  El U2 tomó mucha película.                    \\
A: 5       & \textsc{\small ref:} Nato U2ninra kikin icha película bike. \\
F: 5       & \textsc{\small out:} U2ninra icha pelicula bike.      \\ \hline
C: 48.3 & \textsc{\small src:} No teníamos televisión.                    \\
A: 5       & \textsc{\small ref:} Noara televisiónma ika iki. \\
F: 5       & \textsc{\small out:} Televisiónmara noa iwanke.      \\ \hline
\end{tabular}
}
\caption{Translation outputs of the best system (\texttt{Helsinki}) for Shipibo-Konibo. Top-3 samples have the highest ChrF (C) scores, whereas the bottom-3 have the best adequacy (A) and fluency (F) values.}
\label{tab:shp-samples}
\end{table}


\begin{table}[]
\setlength\tabcolsep{2.5pt}
\resizebox{\linewidth}{!}{%
\begin{tabular}{lp{9cm}}
Scores     & Sentences                     \\ \hline \hline
C: 49.6 & \textsc{\small src:}  Locust Hill oh claro, sí, genial                   \\
A: 1       & \textsc{\small ref:} Locust Hill handa hâ \\
F: 4       & \textsc{\small out:} Locust Hill ohbu̱ho̱ jä'i      \\ \hline
C: 42.2 & \textsc{\small src:} Kennedy habló con los pilotos.                  \\
A: 4       & \textsc{\small ref:} Kennedy bi ñama nen ya pilotos. \\
F: 3       & \textsc{\small out:} Kennedy bi ñäui ya pihnyo.      \\ \hline
C: 32.2 & \textsc{\small src:} ¿Te gustan los libros de Harry Potter o no?                  \\
A: 4       & \textsc{\small ref:} ¿ di ho-y ya ynttothoma on Harry Potter a hin?  \\
F: 3       & \textsc{\small out:} ¿ Gi pe̱fihu̱ na rä libro ra Harry Potter o hina?      \\ \hline \hline

C: 13.1 & \textsc{\small src:} Un niño murió de los cinco.                   \\
A: 5       & \textsc{\small ref:} nā mehtzi bidû on ya qⴘda \\
F: 5       & \textsc{\small out:} N'a ra bätsi bi du ko ya ku̱t'a.      \\ \hline
C: 13.9 & \textsc{\small src:}  Él recibe ayuda con sus comidas y ropa.                     \\
A: 4       & \textsc{\small ref:} nⴘa di hiâni mâhte nen ynu ynñuni xi ȥáhxo \\
F: 4       & \textsc{\small out:} Nu'a hä häni ko ya hñuni ne ya dutu.      \\ \hline
C: 13.3 & \textsc{\small src:} Ni siquiera entendió la ceremonia nupcial, ni siquiera sabía que se había casado, en serio--                    \\
A: 4       & \textsc{\small ref:} Hin bi ô̮ccode na nînthadi, hin mipâca guê bin miqha nthâdi,maqhuani ngu -a. \\
F: 4       & \textsc{\small out:} Inbi bädi te ra nge'a bi ntha̱ti, bi o̱t'e ra gue̱nda...      \\ \hline
\end{tabular}
}
\caption{Translation outputs of the best system (\texttt{Helsinki}) for Otom\'i. Top-3 samples have the highest ChrF (C) scores, whereas the bottom-3 have the best adequacy (A) and fluency (F) values.}
\label{tab:oto-samples}
\end{table}

% ratio Spanish words in L
% OOV ratio
% What about the morphological complex words?
% Orthographic problems (char sets? output vs reference)

\section{Conclusion}
\label{sec:conclusions}

This paper presents the results of the AmericasNLP 2021 Shared Task on OMT. We received 214 submissions %large variety 
of machine translation systems by 8 teams. All systems suffered from the minimal amount of data and the challenging orthographic, dialectal and domain mismatches of the training and test set. However, most teams achieved huge improvements over the official baseline. We found that text cleaning and normalization, as well as domain adaptation played large roles in the best performing systems. The best NMT systems were multilingual approaches with a limited size (over massive multilingual). Additionally, SMT models also performed well, outperforming larger pretrained submissions. 

%For the next edition of our shared task, we want to extend the coverage of languages, as well add human evaluation to the shared task metrics.

\section*{Acknowledgments}

We would like to thank translators of the test and development set, that made this shared task possible: 
Francisco Morales (Bribri), Feliciano Torres Ríos and Esau Zumaeta Rojas  (Asháninka), Perla Alvarez Britez (Guarani), Silvino González de la Crúz (Wixarika), Giovany Martínez Sebastián, Pedro Kapoltitan, and José Antonio (Nahuatl), José Mateo Lino Cajero Velázquez (Otomí), Liz Chávez (Shipibo-Konibo), and María del Cármen Sotelo Holguín (Rarámuri). We also thank our sponsors for their financial support: Facebook AI Research, Microsoft Research, Google Research, the Institute of Computational Linguistics at the University of Zurich, the NAACL Emerging Regions Funding, Comunidad Elotl, and Snorkel AI. Additionally we want to thank all participants for their submissions and effort to advance NLP research for the indigenous languages of the Americas. Manuel Mager received financial support by DAAD Doctoral Research Grant for this work.

